Mini-batch stochastic three-operator splitting for distributed optimization

We consider a network of agents, each with its own private cost consisting of a sum of two possibly nonsmooth convex functions, one of which is composed with a linear operator. At every iteration each agent performs local calculations and can only communicate with its neighbors. The challenging aspect of our study is that the smooth part of the private cost function is given as an expected value and agents only have access to this part of the problem formulation via a heavy-tailed stochastic oracle. To tackle such sampling-based optimization problems, we propose a stochastic extension of the triangular pre-conditioned primal-dual algorithm. We demonstrate almost sure convergence of the scheme and validate the performance of the method via numerical experiments.

==> BlockExtension.tex <==
%----------------------------------------------------------------------
%%% Block
%----------------------------------------------------------------------
% !TEX root = ./StochasticTRIPD.tex

In this section we describe a randomized block coordinate descent version of STripD. We assume that there is a partitioning of the primal--dual variables in $m$ blocks. Let $\scrZ_{i}=\scrH_{i}\oplus\scrG_{i},1\leq i\leq m$. A generic element of block $\scrZ_{i}$ is denoted as $(y^{i},x^{i})$. To perform a general block coordinate descent analysis, let $(\scrZ_{i})_{1\leq i\leq m}$ be separable real Hilbert spaces and let $\scrZ=\scrZ_{1}\oplus\ldots\oplus\scrZ_{m}$ be their direct Hilbert sum. Let $\scrD=\{0,1\}^{m}\setminus\{\0_{m}\}$ and $\eps_{k}=(\eps^{1}_{k},\ldots,\eps^{N}_{k})$ be a binary random vector composed of iid Bernoulli random variables $\eps^{i}_{k}\sim\Ber(p_{i})$ for all $i=1,\ldots,m$ such that $p_{i}\geq 0$. For each block $i\in\{1,\ldots,m\}$ we are give a sequence of maps $T^{i}_{k}:\scrZ\to\scrZ_{i}$ representing an underlying deterministic evolution acting on the $i$-th block. This deterministic map is not directly accessible, but rather can be simulated by means of a sequence of measurable functions $\T^{i}_{k}:\scrZ\times\Omega\to\scrZ_{i}$. This leads to the update of block $i$ as 
\begin{equation}
Z^{i}_{k+1}(\omega)=Z^{i}_{k}(\omega)+\eps^{i}_{k}\left(\T^{i}_{k}(Z_{k},\omega)-Z^{i}_{k}(\omega)\right),
\end{equation}
for all $i=1,\ldots,m,k\geq 0.$
Once this is done for each activated block, we can perform to collective update $Z_{k+1}=[Z^{1}_{k+1},\ldots,Z^{N}_{k+1}]$. This defines a random sweeping method in the spirit of \cite{ComPes15}, summarized below. 
%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}[h!]
\caption{Block coordinate STriPD algorithm}
\label{alg:BSTriPD}
\SetAlgoLined
\KwData{$x_{0}\in\scrH,y_{0}\in\scrG$}
\While{$k=0,\dots,$}
{Realize $\eps_{k}=(\eps^{1}_{k},\ldots,\eps_{k}^{N}),\eps^{i}_{i}\sim\Ber(p_{i})$ i.i.d\;
For all $i\in\{1,\ldots,m\}$ 
\begin{align*}
Z^{i}_{k+1}=Z^{i}_{k}+\eps^{i}_{k}\left(\T^{i}_{k}(Z_{k})-Z^{i}_{k}\right).
\end{align*}
}
\end{algorithm}
%%%%%%%%%%%%%%%%%%%%%%%%%

To analyze the evolution of the Markov chain $(Z_{k})_{k\geq 0}$, let us introduce the auxiliary variable 
\begin{equation}
\tilde{Z}^{i}_{k+1}=\T^{i}_{k}(Z_{k}), \quad \tilde{Z}_{k}=[\tilde{Z}^{1}_{k},\ldots,\tilde{Z}^{N}_{k}],
\end{equation}
which would correspond the collection of random variables when all blocks are updated in parallel. The Markov chain $(Z_{k})_{k\geq 0}$ is then realized as the block-coordinate update 
\[
Z^{i}_{k+1}=Z^{i}_{k}+\eps^{i}_{k}(\tilde{Z}^{i}_{k+1}-Z^{i}_{k})\qquad\forall i\in\{1,\ldots,m\},k\geq 0.
\]
Given a collection of positive operators $\bS_{i}\in\scrP_{\alpha_{i}}(\scrZ_{i})$, we define on $\scrZ$ the norm 
\begin{equation}
(\forall z\in\scrZ):\norm{z}_{\scrZ}\eqdef\sqrt{\sum_{i=1}^{m}\frac{1}{p_{i}}\norm{z^{i}}_{\bS_{i}}^{2}}.
\end{equation}
For the convergence analysis of Algorithm \ref{alg:BSTriPD} we make the following structural assumption on the stochastic generator of block $i\in\{1,\ldots,m\}$. Let $\setS=\bigcap_{k\in\N}\Fix(T_{k})$. 
%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{ass:structural}
There are non-negative stochastic process $(a^{i}_{k})_{k},(b_{k}^{i})_{k}$ such that $b^{i}_{k}\in\ell^{1}_{+}(\F)$ and 
\begin{equation}
\Ex_{k}\left[\norm{\T^{i}_{i}(Z_{k})-z^{\ast}_{i}}^{2}_{\bS_{i}}\right]\leq \norm{Z^{i}_{k}-z^{\ast}_{i}}^{2}_{\bS_{i}}+a^{i}_{k}-b^{i}_{k}\quad\text{a.s.}
\end{equation}
for all $i=1,\ldots,m$ and $k\in\N$ and $z^{\ast}\in\setS$.
\end{assumption}
%%%%%%%%%%%
We will see that this assumption is naturally satisfied by the block implementations on STRiPD. 

\begin{theorem}
Consider Algorithm \ref{alg:BSTriPD} under Assumption \ref{ass:structural}. Set $\scrE_{k}=\sigma(\eps_{k})$ and let $(\scrA_{k})_{k}$ be the filtration defined by $\scrA_{k}=\sigma(Z_{1},\ldots,Z_{k})$. Assume that 
\begin{itemize}
\item[(i)] $\setS=\bigcap_{k\in\N}\Fix(T_{k})\neq\emptyset$, where $T_{k}(z)=(T^{1}_{k}(z),\ldots,T^{N}_{k}(z))$;
\item[(ii)] For every $k\in\N$, the sub-sigma algebras $\scrE_{k}$ and $\scrA_{k}$ are independent;
\item[(iiii)] $p_{i}=\Pr(\eps_{i,k}=1)=\Ex(\eps_{i,k})>0$ for all $i\in\{1,\ldots,m\}$ and $k\in\N$.
\end{itemize}
Then, $(Z_{k})_{k\in\N}$ converges almost surely to $\setS$-valued random variable.
\end{theorem}
\begin{proof}
Let $z^{\ast}\in\setS$ be arbitrary. We have 
\begin{align*}
&\Ex_{k}\left[\norm{Z_{k+1}-z^{\ast}}^{2}_{\scrZ}\right]=\sum_{i=1}^{m}\frac{1}{p_{i}}\Ex_{k}\left[\norm{Z^{i}_{k+1}-z^{\ast}_{i}}^{2}_{\bS_{i}}\right]\\
&=\sum_{i=1}^{m}\frac{1}{p_{i}}\Ex_{k}\left[\norm{Z^{i}_{k}+\eps^{i}_{k}(\tilde{Z}^{i}_{k+1}-Z^{i}_{k})-z^{\ast}_{i}}^{2}_{\bS_{i}}\right]\\
&=\sum_{i=1}^{m}\Ex_{k}\left[\norm{\tilde{Z}^{i}_{k+1}-z^{\ast}_{i}}^{2}_{\bS_{i}}\right]+\sum_{i=1}^{m}\frac{1-p_{i}}{p_{i}}\Ex_{k}\left[\norm{Z^{i}_{k}-z^{i}_{\ast}}^{2}_{\bS_{i}}\right].
\end{align*}
To each block of the process $\tilde{Z}_{k}$ we apply Assumption \ref{ass:structural}, to obtain 

\begin{align*}
\Ex_{k}\left[\norm{Z_{k+1}-z^{\ast}}^{2}_{\scrZ}\right]\leq \norm{Z_{k}-z^{\ast}}^{2}_{\scrZ}+\sum_{i=1}^{m}(a^{i}_{k}-b_{k}^{i}).
\end{align*}
The convergence follows from the Robbins-Siegmund Lemma.
\end{proof}

%\begin{align*}
%\norm{\tilde{Z}^{i}_{k+1}-z^{i}_{\ast}}^{2}_{\bS_{i}}&\leq \norm{Z^{i}_{k}-z^{i}_{\ast}}^{2}_{\bS_{i}}+\left(\mu_{i}\frac{1-\alpha}{\alpha}\frac{1+\sigma_{i}^{2}M(L_{i}^{\ast}L_{i})}%{\gamma_{i}}+2\right)\Ex_{k}[\nu^{i}_{k}]\\
%&-\mu(1-\alpha)\norm{T^{i}_{k}(Z_{k})-Z^{i}_{k}}^{2}.
%\end{align*}
%Since $\Ex_{k}\nu^{i}_{k}=\frac{\sigma(X_{k})^{2}}{N_{k}}$, it follows 
%\begin{align*}
%\Ex_{k}\left[\norm{Z_{k+1}-z^{\ast}}^{2}_{\scrZ}\right]&\leq \norm{Z_{k}-z^{\ast}}^{2}_{\scrZ}+a_{k}-b_{k}
%\end{align*}
%with $(a_{k})\in\ell^{1}_{+}(\Pr)$. Therefore $b_{k}\to 0$ a.s and the convergence result follows. 





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Structured Convex Optimization}
As a concrete example, we are motivated by solving block-decomposed convex optimization problems of the form 
\begin{equation}
\min_{x\in\scrH}f(x)+\sum_{i=1}^{N}(g_{i}(x^{i})+h_{i}(L_{i}x^{i})).
\end{equation}
In this problem, the coupling between primal and dual variables is carried with the function $f(x^{(1)},\ldots,x^{(N)})$, which is given as an expected value 
\begin{equation}
f(x^{1},\ldots,x^{N})\eqdef\Ex[\hat{f}(x^{1},\ldots,x^{N},\xi)],\quad\xi\sim\measP. 
\end{equation}
Let $Lx=[L_{1}x^{1},\ldots,L_{m}x^{m}]$, where each $L_{i}\in\scrB(\scrH_{i},\scrG_{i})$. Given scalars $\sigma_{i},\gamma_{i}>0$, define 
\begin{align}
\bS_{i}(y_{i},x_{i})&=\left[\frac{1}{\sigma_{i}}y_{i},\frac{1}{\gamma_{i}}x_{i}\right],\\
\bP_{i}(y_{i},x_{i})&=\left[\frac{1}{\sigma_{i}}y_{i}+\frac{1}{2}L_{i},\frac{1}{2}L_{i}^{\ast}y_{i}+\frac{1}{\gamma_{i}}x_{i}\right],\\
\bK_{i}(y_{i},x_{i})&=\left[-\frac{1}{2}L_{i}x_{i},\frac{1}{2}L^{\ast}_{i}y_{i}\right].
\end{align}
Finally, define the operator 
\[
\bR_{i}(y_{i},x_{i})=\left[\frac{1}{\sigma_{i}}y_{i},L_{i}^{\ast}y_{i}+\frac{1}{\gamma_{i}}x_{i}\right].
\]
Let us introduce the block-specific operators
\begin{align}
&\setA_{i}(y^{i},x^{i})\eqdef\partial h^{\ast}_{i}(y^{i})\times\partial g_{i}(x^{i}),\\
&\setM_{i}(y^{i},x^{i})\eqdef[-L_{i}x^{i},L^{\ast}_{i}y^{i}],\\
&\setC_{i}(y,x)\eqdef[0,\nabla^{(i)} f(x)], \text{where }\nabla^{(i)}f(x)\eqdef\frac{\partial}{\partial x_{i}}f(x)
\end{align}

\begin{remark}
Instead of scalar-valued step sizes, we could have chosen more general block-specific positive operators $\Sigma_{i},\Gamma_{i}$. This would lead to no new insights, at the cost of more complex notation, and thus we prefer not to do this extension here.
\end{remark} 

We are going to construct a stochastic process $Z_{k}=[Z^{1}_{k},\ldots,Z^{m}_{k}]$ as a discrete-time Markov chain on the Hilbert space $\scrZ$. To that end, let us introduce the stochastic sequence $(\hat{Z}^{i}_{k})_{k\geq 0}$ by 
\begin{equation}
0\in (\bR_{i}+\setA_{i})(\hat{Z}^{i}_{k})-(\bR_{i}-\setM_{i})(Z^{i}_{k})-\hat{\scrC}_{i,k}(Z_{k})
\end{equation}
In coordinates $\hat{Z}^{i}_{k}=(\hat{Y}^{i}_{k},\hat{X}^{i}_{k})$, this reads as
\begin{align}
&\hat{Y}^{i}_{k}=\prox_{\sigma_{i}h_{i}^{\ast}}(Y^{i}_{k}+\sigma_{i}L_{i}X^{i}_{k}),\\
&\hat{X}^{i}_{k}=\prox_{\gamma_{i}g_{i}}(X^{i}_{k}-\gamma_{i}\scrF^{i}_{k}(X_{k})-\gamma_{i}L_{i}^{\ast}Y^{i}_{k}).
\end{align}
Define the mapping $\T_{i}:\scrZ\times\Omega\to\scrZ_{i}$ by 
\begin{equation}\label{eq:Ti}
\T_{i}(Z_{k},\omega)\eqdef[ \hat{Y}^{i}_{k}(\omega)+\sigma_{i}L_{i}(\hat{X}^{i}_{k}(\omega)-X^{i}_{k}),\hat{X}_{k}^{i}(\omega)].
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{remark}
The random block stochastic gradient method STriPD is flexible in terms of the block-activation strategy chosen. 
\begin{itemize}
\item Mulit-block activation: at each iteration the $j$-th block is activated with probability $p_{j}>0$ independent of other blocks. 
\item Single-block activation: At each iteration, on coordinate block is selected. This can be achieved by adding the restriction $\sum_{i=1}^{m}p_{i}=1$ to the sampling mechanism. 
\end{itemize}
\end{remark}

For the convergence of the resulting block algorithm, we just note that 

\begin{align*}
\norm{\tilde{Z}^{i}_{k+1}-z^{i}_{\ast}}^{2}_{\bS_{i}}&\leq \norm{Z^{i}_{k}-z^{i}_{\ast}}^{2}_{\bS_{i}}\\
&+\left(\mu_{i}\frac{1-\alpha}{\alpha}\frac{1+\sigma_{i}^{2}M(L_{i}^{\ast}L_{i})}{\gamma_{i}}+2\right)\Ex_{k}[\nu^{i}_{k}]\\
&-\mu(1-\alpha)\norm{T^{i}_{k}(Z_{k})-Z^{i}_{k}}^{2}.
\end{align*}\BFnote{we haven't introduced mini-batches}
Since $\Ex_{k}[\nu^{i}_{k}]=\frac{\sigma(X_{k})^{2}}{N_{k}}$, we can set 
\begin{align*}
a^{i}_{k}&= \left(\mu_{i}\frac{1-\alpha}{\alpha}\frac{1+\sigma_{i}^{2}M(L_{i}^{\ast}L_{i})}{\gamma_{i}}+2\right)\Ex_{k}[\nu^{i}_{k}],\text{ and }\\
b^{i}_{k}&=\mu(1-\alpha)\norm{T^{i}_{k}(Z_{k})-Z^{i}_{k}}^{2}
\end{align*}
to end up with
\begin{align*}
\Ex_{k}\left[\norm{Z_{k+1}-z^{\ast}}^{2}_{\scrZ}\right]&\leq \norm{Z_{k}-z^{\ast}}^{2}_{\scrZ}+a_{k}-b_{k}.
\end{align*}
It is easily seen that $(a_{k})\in\ell^{1}_{+}(\Pr)$. Therefore $b_{k}\to 0$ a.s and the convergence result follows. 


%
%\subsection{Multi-agent optimization}
%The 

